Strategy Complexity of B\"uchi and Transience Objectives in Concurrent Stochastic Games

We study 2-player stochastic games on countable graphs. Players Max and Min seek respectively to maximize and minimize the probability of satisfying the game objective. The B\"uchi objective is to visit a given set of states infinitely often. The Transience objective is to visit no state infinitely often. In B\"uchi games there exist $\varepsilon$-optimal Max strategies that use just a step counter plus 1 bit of public memory. This upper bound holds for all countable graphs, but is a new result even for finite graphs. It is tight, since Max strategies that use just a step counter, or just finite memory, are not sufficient even on finite game graphs. This upper bound follows from a slightly stronger new result: $\varepsilon$-optimal Max strategies for the combined B\"uchi and Transience objective require exactly 1 bit of public memory. Moreover, $\varepsilon$-optimal Max strategies for the Transience objective alone can be chosen as memoryless.

==> macro.tex <==
\newcommand{\N}{\mathbb N}
\newcommand{\Q}{\mathbb Q}
\newcommand{\Z}{\+{Z}}
\newcommand{\R}{\+{R}}
\newcommand{\x}{\times}
\newcommand{\eps}{\varepsilon}
\newcommand{\nat}{\mathbb N}
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\len}[1]{\lvert#1\rvert}
\newcommand{\card}[1]{\abs{#1}}


\newcommand{\eqby}[2][=]{\stackrel{\text{{\tiny{#2}}}}{#1}}
\newcommand{\eqdef}{\eqby{def}}

\newcommand{\reachset}{T}
%
\newcommand{\dist}{\mathcal{D}}
\newcommand{\support}{\mathtt{supp}}




\RequirePackage{xifthen}% provides \isempty test
\newcommand{\reach}[1][]{\mathtt{Reach}\ifthenelse{\isempty{#1}}%
    {}% if #1 is empty
    {(#1)}% if #1 is not empty
}
\newcommand{\reachn}[2]{\mathtt{Reach}_{#1}\ifthenelse{\isempty{#2}}%
    {}% if #1 is empty
    {(#2)}% if #2 is not empty
}
\newcommand{\Buchi}[1][]{\Bu\ifthenelse{\isempty{#1}}%
    {}% if #1 is empty
    {(#1)}% if #1 is not empty
}
\newcommand{\safety}[1][]{\mathtt{Safety}\ifthenelse{\isempty{#1}}%
    {}% if #1 is empty
    {(#1)}% if #1 is not empty
}
\newcommand{\avoid}[1][]{\mathtt{Avoid}\ifthenelse{\isempty{#1}}%
    {}% if #1 is empty
    {(#1)}% if #1 is not empty
}
\newcommand{\tuple}[1]{\lrc{#1}}
\newcommand{\game}{{\mathcal G}}
\newcommand{\mdp}{{\mathcal M}}
\newcommand{\states}{S}
\renewcommand{\state}{s}
\newcommand{\Tr}{\mathtt{Tr}}
\newcommand{\transient}{\Tr}
\newcommand{\Not}{\mathtt{Not}}
\newcommand{\Ret}{\mathtt{Ret}}
\newcommand{\Vis}{\mathtt{Vis}}
\newcommand{\Bu}{\mathtt{Bu}}
\newcommand{\TB}{\mathtt{TB}}
\newcommand{\bev}[1]{\langle #1 \rangle}
\newcommand{\Cyl}[1]{\mathit{Cyl}(#1)}

\newcommand{\transition}{{\longrightarrow}}
\newcommand{\probp}{p}
%
\newcommand{\playset}{E}
\newcommand{\zstrat}{\sigma}
\newcommand{\ostrat}{\pi}
\newcommand{\xstrat}{\tau}
%
\newcommand{\zstratset}{\Sigma}
\newcommand{\ostratset}{\Pi}
\newcommand{\expectval}{{\mathcal E}}
\newcommand{\probm}{{\mathcal P}}
\newcommand{\expectation}[1][]{ \expectval_{#1}}
\newcommand{\valueo}[1]{{\mathtt{val}_{#1}}}
\newcommand{\valueof}[2]{{\mathtt{val}_{#1}(#2)}}
\newcommand{\valueoflower}[2]{{\mathtt{val}^\downarrow_{#1}(#2)}}
\newcommand{\valueofupper}[2]{{\mathtt{val}^\uparrow_{#1}(#2)}}

\newcommand{\weighted}[1]{{\mathcal W}_{#1}}
\newcommand{\sca}[2]{\langle#1,#2\rangle}
% argmin already defined
%\DeclareMathOperator*{\argmin}{arg\,min}

% mahsa
\def\mahsa#1{{\color{green!50!black} $\clubsuit$ Mahsa: #1  \color{black}}}
\def\stefan#1{{\color{blue!90!black} $\clubsuit$ Stefan: #1  \color{black}}}
\def\ste#1{{\color{blue!90!black}#1\color{black}}}


\newcommand{\memconfset}{{\sf M}}
\newcommand{\memory}{{\sf M}}
\newcommand{\updatefun}{u}
\newcommand{\memconf}{{\sf m}}
\newcommand{\memsuc}{\pi_s}
\newcommand{\memtransx}{\memsuc{\px}}
\newcommand{\memup}{\pi_u}



\newcommand{\ptnote}[2][]{\todo[size=\footnotesize,color=blue!20,bordercolor=blue!20,linecolor=blue!20,#1]{PT: #2}}
\newcommand{\sknote}[2][]{\todo[size=\footnotesize,color=red!20,bordercolor=blue!20,linecolor=blue!20,inline,#1]{PT: #2}}
\newcommand{\strategy}{\zstrat}
\newcommand{\stratAct}[1][\strategy]{{#1}_{\mathop{act}\nolimits}}
\newcommand{\stratUp}[1] [\strategy]{{#1}_{\mathop{up}\nolimits}}

\newcommand{\ignore}[1]{}

\newcommand{\mysec}[1]{\subsubsection*{#1}}


% \def\Halmos{\mbox{\quad$\square$}}
% Not needed in ACM 
\def\Halmos{}



==> preamble.tex <==
\RequirePackage{amsmath,amsfonts}
\usepackage{dsfont}
\usepackage{thmtools} 
\usepackage{thm-restate}
\usepackage[capitalize,noabbrev]{cleveref}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{multirow}
\usepackage{caption}

